Redirect2Own: Protecting the Intellectual Property of User-uploaded Content through Off-site Indirect Access

Social networking services have attracted millions of users, including individuals, professionals, and companies, that upload massive amounts of content, such as text, pictures, and video, every day. Content creators retain the intellectual property (IP) rights on the content they share with these networks, however, very frequently they implicitly grant them, a sometimes, overly broad license to use that content, which enables the services to use it in possibly undesirable ways. For instance, Facebook claims a transferable, sub-licensable, royalty-free, worldwide license on all user-provided content. Professional content creators, like photographers, are particularly affected. In this paper we propose a design for decoupling user data from social networking services without any loss of functionality for the users. Our design suggests that user data are kept off the social networking service, in third parties that enable the hosting of user-generated content under terms of service and overall environment (e.g., a different location) that better suit the user's needs and wishes. At the same time, indirection schemata are seamlessly integrated in the social networking service, without any cooperation from the server side necessary, so that users can transparently access the off-site data just as they would if hosted in-site. We have implemented our design as an extension for the Chrome Web browser, called Redirect2Own, and show that it incurs negligible overhead on accessing 'redirected' content. We offer the extension as free software and its code as an open-source project.

==> Makefile <==
BIBTEX=bibtex
PDFLATEX=pdflatex -interaction=nonstopmode --shell-escape

TARGET=photo_ownership

TEXFILES=*.tex
BIBFILES=*.bib
FIGFILES=
EXTRAS=*.cls *.sty *.bst

.PHONY: clean figs

$(TARGET).pdf: $(TEXFILES) $(BIBFILES) $(FIGFILES) $(TARGET).aux
	$(PDFLATEX) $(TARGET).tex
	$(PDFLATEX) $(TARGET).tex

$(TARGET).aux: $(TEXFILES)
	$(PDFLATEX) $(TARGET).tex
	$(BIBTEX) $(TARGET)

figs:
	#$(MAKE) -C figs

zip:
	mkdir -p /tmp/$(TARGET)
	ls -1 $(TEXFILES) | sed 's/^/\.\//' | cpio -dump /tmp/$(TARGET)/
	ls -1 $(BIBFILES) | sed 's/^/\.\//' | cpio -dump /tmp/$(TARGET)/
	ls -1 $(FIGFILES) | sed 's/^/\.\//' | cpio -dump /tmp/$(TARGET)/
	ls -1 $(EXTRAS) | sed 's/^/\.\//' | cpio -dump /tmp/$(TARGET)/
	cd /tmp && rm -f $(TARGET).zip && zip -r $(TARGET).zip $(TARGET)
	mv /tmp/$(TARGET).zip .
	rm -rf /tmp/$(TARGET)


dist:
	mkdir -p /tmp/$(TARGET)
	ls -1 $(TEXFILES) | sed 's/^/\.\//' | cpio -dump /tmp/$(TARGET)/
	ls -1 $(BIBFILES) | sed 's/^/\.\//' | cpio -dump /tmp/$(TARGET)/
	ls -1 $(FIGFILES) | sed 's/^/\.\//' | cpio -dump /tmp/$(TARGET)/
	ls -1 $(EXTRAS) | sed 's/^/\.\//' | cpio -dump /tmp/$(TARGET)/
	cd /tmp && rm -f $(TARGET).tar.gz && \
		tar -cf - $(TARGET) | gzip > $(TARGET).tar.gz
	mv /tmp/$(TARGET).tar.gz .
	rm -rf /tmp/$(TARGET)


clean:
	rm -f *.aux *.bbl *.blg *.log *.dvi *.toc *.lof \
		$(TARGET).pdf *.out *.idx *.ent *.ind *.ilg
	make -C figs clean

